Proof Nets, Coends and the Yoneda Isomorphism

Proof nets provide permutation-independent representations of proofs and are used to investigate coherence problems for monoidal categories. We investigate a coherence problem concerning Second Order Multiplicative Linear Logic (MLL2), that is, the one of characterizing the equivalence over proofs generated by the interpretation of quantifiers by means of ends and coends. We provide a compact representation of proof nets for a fragment of MLL2 related to the Yoneda isomorphism. By adapting the "rewiring approach" used in coherence results for star-autonomous categories, we define an equivalence relation over proof nets called "re-witnessing". We prove that this relation characterizes, in this fragment, the equivalence generated by coends.

==> eptcsdata.tex <==
\providecommand{\firstpage}{148}
\providecommand{\publicationstatus}{T. Ehrhard, M. Fern\'andez, V. de Paiva, L. Tortora de Falco (Eds.):\\ Linearity-TLLA 2018\\
EPTCS 292, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.292.9}{10.4204/EPTCS.292.9}}

